Trustworthy Machine Learning under Distribution Shifts

Machine Learning (ML) has been a foundational topic in artificial intelligence (AI), providing both theoretical groundwork and practical tools for its exciting advancements. From ResNet for visual recognition to Transformer for vision-language alignment, the AI models have achieved superior capability to humans. Furthermore, the scaling law has enabled AI to initially develop general intelligence, as demonstrated by Large Language Models (LLMs). To this stage, AI has had an enormous influence on society and yet still keeps shaping the future for humanity. However, distribution shift remains a persistent ``Achilles' heel'', fundamentally limiting the reliability and general usefulness of ML systems. Moreover, generalization under distribution shift would also cause trust issues for AIs. Motivated by these challenges, my research focuses on \textit{Trustworthy Machine Learning under Distribution Shifts}, with the goal of expanding AI's robustness, versatility, as well as its responsibility and reliability. We carefully study the three common distribution shifts into: (1) Perturbation Shift, (2) Domain Shift, and (3) Modality Shift. For all scenarios, we also rigorously investigate trustworthiness via three aspects: (1) Robustness, (2) Explainability, and (3) Adaptability. Based on these dimensions, we propose effective solutions and fundamental insights, meanwhile aiming to enhance the critical ML problems, such as efficiency, adaptability, and safety.

==> src/publication.tex <==
\chapter*{List of Publications}
All of the works described in this thesis have been previously published or under review during my PhD, which includes:
\begin{itemize}
    \item[(1)] \textbf{Zhuo Huang}, Xiaobo Xia, Li Shen, Bo Han, Mingming Gong, Chen Gong, Tongliang Liu. ``Harnessing Out-Of-Distribution Examples via Augmenting Content and Style''. In \textit{ICLR}, 2023.


    \item[(2)] \textbf{Zhuo Huang}, Miaoxi Zhu, Xiaobo Xia, Li Shen, Jun Yu, Chen Gong, Bo Han, Bo Du, Tongliang Liu. ``Robust Generalization against Photon-Limited Corruptions via Worst-Case Sharpness Minimization''. In \textit{CVPR}, 2023.

    
    \item[(3)] \textbf{Zhuo Huang}, Li Shen, Jun Yu, Bo Han, Tongliang Liu. ``FlatMatch: Bridging Labeled Data and Unlabeled Data with Cross-Sharpness for Semi-Supervised Learning''. In \textit{NeurIPS}, 2024.

    
    \item[(4)] \textbf{Zhuo Huang}, Muyang Li, Li Shen, Jun Yu, Chen Gong, Bo Han, Tongliang Liu. ``Winning Prize Comes from Losing Tickets: Improve Invariant Learning by Exploring Variant Parameters for Out-of-Distribution Generalization''. In \textit{IJCV}, 2024.

    
    \item[(5)] \textbf{Zhuo Huang}, Chang Liu, Yinpeng Dong, Hang Su, Shibao Zheng, Tongliang Liu. ``Machine Vision Therapy: Multimodal Large Language Models Can Enhance Visual Robustness via Denoising In-Context Learning''. In \textit{ICML}, 2024.

    
    \item[(6)] \textbf{Zhuo Huang}, Gang Niu, Bo Han, Masashi Sugiyama, Tongliang Liu. ``Towards Out-of-Modal Generalization without Instance-level Modal Correspondence''. In \textit{ICLR}, 2025.

    
    \item[(7)] \textbf{Zhuo Huang}, Runnan Chen, Bo Han, Gang Niu, Masashi Sugiyama, Tongliang Liu. ``BrokenBind: Universal Modality Exploration Beyond Dataset Boundaries''. Under review, 2025.

    
    \item[(8)] \textbf{Zhuo Huang}, Qizhou Wang, Ziming Hong, Shanshan Ye, Bo Han, Tongliang Liu. ``Memorize to Forget: Machine Unlearning without Gradient Ascent via Model Extrapolation''. Under review, 2025.

    
    \item[(9)] Haoyu Wang, \textbf{Zhuo Huang}, Zhiwei Lin, Tongliang Liu. ``NoiseGPT: Label Noise Detection and Rectification through Probability Curvature''. In \textit{NeurIPS}, 2025.


    \item[(10)] Puning Yang, Qizhou Wang, \textbf{Zhuo Huang}, Tongliang Liu, Chengqi Zhang, Bo Han. ``Exploring Criteria for Enhanced Loss Reweighting in Large Language Model Unlearning''. In \textit{ICML}, 2025.


    \item[(11)] Xiaohao Liu, Xiaobo Xia, \textbf{Zhuo Huang}, Tat-Seng Chua. ``Towards Modality Generalization: A Benchmark and Prospective Analysis''. In \textit{ACM MM}, 2025.

    
    \item[(12)] Ziming Hong, Zhenyi Wang, Li Shen, Yu Yao, \textbf{Zhuo Huang}, Shiming Chen, Chuanwu Yang, Mingming Gong, Tongliang Liu. ``Improving Non-Transferable Representation Learning by Harnessing Content and Style''. In \textit{ICLR}, 2024.
    
\end{itemize}
